Dynamics of solar Coronal Mass Ejections: forces that impact their propagation

We investigate the Sun-Earth dynamics of a set of 38 well-observed Coronal Mass Ejections(CMEs) using data from the STEREO, SOHO missions and WIND instrument. We seek to quantify the relative contributions of Lorentz force and aerodynamic drag on their propagation. The CMEs are 3D reconstructed using the Graduated Cylindrical Shell(GCS) model to derive observed CME parameters.Using a microphysical prescription of the drag coefficient,we find that solar wind aerodynamic drag adequately accounts for the dynamics of the fastest CMEs from as low as 3.5 Rs. For relatively slower CMEs, however, we find that when the drag-based model is initiated below the distances ranging from 12 to 50 Rs,the observed CME trajectories cannot be accounted for.This suggests that aerodynamic drag force dominates the dynamics of slower CMEs only above these heights.To investigate CME dynamics below the heights where aerodynamic drag dominates, we consider the Torus Instability model for the driving Lorentz force. We find that for fast CMEs,Lorentz forces become negligible in comparison to aerodynamic drag as early as 3.5-4 Rs.For slow CMEs, however, they become negligible only by 12-50 Rs.This justifies the success of the drag-only model for fast CMEs. In case of slow CMEs, the Lorentz force is only slightly smaller than the drag force even beyond 12-50 Rs.For these slow events,our results suggest that some of the magnetic flux carried by CMEs might be expended in expansion or heating. These dissipation effects might be important in describing the propagation of slower CMEs. To the best of our knowledge,this is the first systematic study in this regard using a diverse CME sample. A physical understanding of the forces that affect CME propagation and how they compare with each other at various heliocentric distances is an important ingredient in building tools for describing and predicting CME trajectories.

==> preamble.tex <==
%% THE PREAMBLE: Packages and Page Setup
%%
\usepackage{graphicx}
\usepackage{longtable,lscape}
\usepackage{hyperref}
%\usepackage[landscape]{geometry}
%\usepackage{color}
\usepackage{cite} % for range of numbers in cite - Resmi
%\usepackage{graphicx}% Include figure files
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{amsmath}%this is needed for sub-equations - Resmi
\usepackage{amssymb}
\usepackage{bm}% bold math
\usepackage{makeidx}% for making index
\usepackage{setspace}%for adjusting the line spacing - Resmi
%\setlength{\parskip}{10pt plus 1pt minus 1pt}
\usepackage{mathrsfs}
\usepackage[T1]{fontenc}
\usepackage{lmodern}

\makeindex

